A discretize-then-map approach for the treatment of parameterized geometries in model order reduction

We present a general approach for the treatment of parameterized geometries in projection-based model order reduction. During the offline stage, given (i) a family of parameterized domains $\{ \Omega_{\mu}: \mu \in \mathcal{P} \} \subset \mathbb{R}^D$ where $\mu \in \mathcal{P} \subset \mathbb{R}^P$ denotes a vector of parameters, (ii) a parameterized mapping ${\Phi}_{\mu}$ between a reference domain $\Omega$ and the parameter-dependent domain $\Omega_{\mu}$, and (iii) a finite element triangulation of $\Omega$, we resort to an empirical quadrature procedure to select a subset of the elements of the grid. During the online stage, we first use the mapping to "move" the nodes of the selected elements and then we use standard element-wise residual evaluation routines to evaluate the residual and possibly its Jacobian. We discuss how to devise an online-efficient reduced-order model and we discuss the differences with the more standard "map-then-discretize" approach (e.g., Rozza, Huynh, Patera, ACME, 2007); in particular, we show how the discretize-then-map framework greatly simplifies the implementation of the reduced-order model. We apply our approach to a two-dimensional potential flow problem past a parameterized airfoil, and to the two-dimensional RANS simulations of the flow past the Ahmed body.

==> imm/graphical_abstract.tex <==
\begin{tikzpicture}[scale=5]
\linethickness{0.3 mm}
\begin{scope}[yshift=0.3cm]
\draw[ultra thick]  (0.1,0.05)--(1.044,0.05)--(1.044,0.2442)--(0.8428,0.3380)--(0.1,0.3380);
\draw [ultra thick,domain=90:180,samples=300] plot ({0.1+0.1*cos(\x)}, {0.2380+0.1*sin(\x)});
\draw [ultra thick,domain=180:270,samples=300] plot ({0.1+0.1*cos(\x)}, {0.15+0.1*sin(\x)});
\draw[ultra thick]  (0,0.2380)--(0,0.1500);

\draw [blue,ultra thick,dashed,domain=335:360,samples=30] plot ({0.8428+0.2*cos(\x)}, {0.3380+0.2*sin(\x)});
\draw[blue,dashed,ultra thick]  (0.8428,0.3380)--(1.0428,0.3380);
 \coordinate [label={right:  {\Large{$\mu$}}}] (E) at (1.0428,0.3) ;
  
\draw[ultra thick]  (-0.2,0)--(1.2,0); 
 \draw[<->]  (1.1,0)--(1.1,0.05); 
  \coordinate [label={right:  {{$h_{\rm b}$}}}] (E) at (1.1,0.05) ;

  \draw[<->]  (0,0.4)--(1.044,0.4); 
  \coordinate [label={above:  {{$L$}}}] (E) at (0.522,0.4) ;

\draw[<->]  (1.2,0.05)--(1.2,0.3380); 
  \coordinate [label={right:  {{$H_{\rm c}$}}}] (E) at (1.2,0.17) ;
 
\draw[<->]  (0.8428-0.02,0.3380-0.02)--(1.044-0.02,0.2442-0.02);  
   \coordinate [label={below:  {{$\delta$}}}] (E) at (0.9234, 0.2711) ;
 
 \draw[<->]  (0.1,0.15)--(0,0.15);  
   \coordinate [label={above:  {{$R$}}} ] (E) at (0.05, 0.15) ;
   \end{scope}
   
 \coordinate [label={above:  {\textcolor{white}{0}} } ] (E) at (0,0) ;  
   
   
\end{tikzpicture}
~~~
\begin{tikzpicture}[scale=0.7]
\begin{semilogyaxis}[
  %title = {Convergence Plot},
xlabel = {ROM dimension},
  ylabel = {Relative error},
  %legend entries = {$d=2$, $d=3$, $d = 4$},
  line width=1.2pt,
  mark size=3.0pt,
  ymin=0.00001,   ymax=0.05,
 % legend style={at={(0,0)},anchor=south west}
  ]
    \addplot[line width=1.pt,color=black,mark=o] table {data/RANS/Re3e3/proj.dat};
    \addplot[line width=1.pt,color=violet,mark=diamond] table {data/RANS/Re3e3/tolm14.dat}; 
     \addlegendentry{Proj error};
      \addlegendentry{ROM error};
\end{semilogyaxis}
\end{tikzpicture}

\includegraphics[width=0.6\textwidth]
{imm/rans/picture_rans.eps}
~
%\hspace{2.95in}
\begin{tikzpicture}[scale=0.7]
\begin{axis}[
  %title = {Convergence Plot},
xlabel = {\LARGE {ROM dimension}},
  ylabel = {\LARGE {$\%$ sampled elements}},
  %legend entries = {$d=2$, $d=3$, $d = 4$},
  line width=1.2pt,
  mark size=3.0pt,
 ymin=0,   ymax=2,
 % legend style={at={(0,0)},anchor=south west}
  ]
 \addplot[line width=1.pt,color=violet,mark=diamond] table {data/RANS/Re3e3/EQtolm14.dat}; 
\end{axis}
 \end{tikzpicture}




==> imm/laplace/performancePG.tex <==
\subfloat[ ] {
\begin{tikzpicture}[scale=0.9]
\begin{semilogyaxis}[
  %title = {Convergence Plot},
xlabel = {$N$},
  ylabel = {$E_{\rm avg}$ },
  %legend entries = {$d=2$, $d=3$, $d = 4$},
  line width=1.2pt,
  mark size=3.0pt,
  ymin=0.00001,   ymax=0.05,
 % legend style={at={(0,0)},anchor=south west}
  ]
    \addplot[line width=1.pt,color=black,mark=o] table {data/laplace/pgal/proj.dat};%\label{ROMperformance:proj_error}
     \addplot[line width=1.pt,color=magenta,mark=square]  table {data/laplace/pgal/hf_quad.dat};%\label{ROMperformance:hf_quad}
  \addplot[line width=1.pt,color=red,mark=square]  table {data/laplace/pgal/tolm6.dat};
  %\label{ROMperformance:tol1em6}
  \addplot[line width=1.pt,color=blue,mark=triangle*] table {data/laplace/pgal/tolm10.dat};
    \addplot[line width=1.pt,color=cyan,mark=diamond] table {data/laplace/pgal/tolm14.dat};
  \label{ROMperformance:tol1em14}
  
  
  %\label{ROMperformance:tol1em10}
  
\end{semilogyaxis}

\end{tikzpicture}
}
~~~
\subfloat[ ] {
\begin{tikzpicture}[scale=0.9]
\begin{axis}[
  %title = {Convergence Plot},
xlabel = {$N$},
  ylabel = {$Q$ },
  %legend entries = {$d=2$, $d=3$, $d = 4$},
  line width=1.2pt,
  mark size=3.0pt,
 ymin=1,   ymax=220,
 % legend style={at={(0,0)},anchor=south west}
  ]
   \addplot[line width=1.pt,color=red,mark=square]  table {data/laplace/pgal/EQtolm6.dat};
  \addplot[line width=1.pt,color=blue,mark=triangle*] table {data/laplace/pgal/EQtolm10.dat};  
    \addplot[line width=1.pt,color=cyan,mark=diamond] table {data/laplace/pgal/EQtolm14.dat};  
 \end{axis}

\end{tikzpicture}
}

% In order to have the same mark size as in the figure
%\bgroup% compute size of \ref in ex
%\sbox0{\ref{data}}%
%\pgfmathparse{\ht0/1ex}%
%\xdef\refsize{\pgfmathresult ex}%
%\egroup

 

==> imm/laplace/residualPG.tex <==
\subfloat[ ] {
\begin{tikzpicture}[scale=0.6]
\begin{axis}[
xlabel = {$N$},
  ylabel = {$J_{\rm r}$ },
  line width=1.2pt,
  mark size=3.0pt,
  ymin=1,   ymax=30
%legend style={at={(0,0)},anchor=south west}
  ]
  \addplot[line width=1.pt,color=red,mark=square]  table {data/laplace/pgal/Jresm6.dat};
  %\label{ROMperformance:tol1em6}
  \addplot[line width=1.pt,color=blue,mark=triangle*] table {data/laplace/pgal/Jresm12.dat};
    \addplot[line width=1.pt,color=cyan,mark=diamond] table {data/laplace/pgal/Jresm14.dat};
 
  
\end{axis}

\end{tikzpicture}
}
~~~
\subfloat[ ] {
\begin{tikzpicture}[scale=0.6]
\begin{axis}[
% title = {Convergence Plot},
xlabel = {$N$},
  ylabel = {$Q_{\rm r}$ },
% legend entries = {$d=2$, $d=3$, $d = 4$},
  line width=1.2pt,
  mark size=3.0pt,
 ymin=10,   ymax=180,
  legend style={at={(0,0)},anchor=south west}
  ]
 
  \addplot[line width=1.pt,color=red,mark=square]  table {data/laplace/pgal/Qresm6.dat};
  %\label{ROMperformance:tol1em6}
  \addplot[line width=1.pt,color=blue,mark=triangle*] table {data/laplace/pgal/Qresm12.dat};
    \addplot[line width=1.pt,color=cyan,mark=diamond] table {data/laplace/pgal/Qresm14.dat};
 
\end{axis}
\end{tikzpicture}
}
~~~
\subfloat[ ] {
\begin{tikzpicture}[scale=0.6]
\begin{loglogaxis}[
% title = {Convergence Plot},
xlabel = {dual residual},
  ylabel = {$H^1$ rel error},
legend entries = {hf res vs error, estimated res vs error},
  line width=1.2pt,
  mark size=3.0pt,
 ymin=0.00001,   ymax=0.01,
legend style={at={(0.03,0.9)},anchor=west}
  ]
 
  \addplot[only marks,color=red,mark=square]  table {data/laplace/gal/EQres.dat};
  %\addlegendentry{model}
  
  \addplot[only marks,color=blue,mark=triangle*] table {data/laplace/gal/hfres.dat};  
  
\end{loglogaxis}
\end{tikzpicture}
}

% In order to have the same mark size as in the figure
%\bgroup% compute size of \ref in ex
%\sbox0{\ref{data}}%
%\pgfmathparse{\ht0/1ex}%
%\xdef\refsize{\pgfmathresult ex}%
%\egroup

